Rethinking RGB-D Fusion for Semantic Segmentation in Surgical Datasets

Surgical scene understanding is a key technical component for enabling intelligent and context aware systems that can transform various aspects of surgical interventions. In this work, we focus on the semantic segmentation task, propose a simple yet effective multi-modal (RGB and depth) training framework called SurgDepth, and show state-of-the-art (SOTA) results on all publicly available datasets applicable for this task. Unlike previous approaches, which either fine-tune SOTA segmentation models trained on natural images, or encode RGB or RGB-D information using RGB only pre-trained backbones, SurgDepth, which is built on top of Vision Transformers (ViTs), is designed to encode both RGB and depth information through a simple fusion mechanism. We conduct extensive experiments on benchmark datasets including EndoVis2022, AutoLapro, LapI2I and EndoVis2017 to verify the efficacy of SurgDepth. Specifically, SurgDepth achieves a new SOTA IoU of 0.86 on EndoVis 2022 SAR-RARP50 challenge and outperforms the current best method by at least 4%, using a shallow and compute efficient decoder consisting of ConvNeXt blocks.

==> tables/lapi2i.tex <==
\begin{table}[h]
\centering
\caption {\textbf{LapI2I Semantic Segmentation}. }
\label{tab:lapi2i} 
\resizebox{0.99\textwidth}{!}{%
\begin{tabular}{c|c|c|c|c}
\hline

\hline

\hline
Methods  & Architecture &  Input size & Pre-train  & IoU \\
\hline

\hline

\hline
MaskRCNN    & ResNet-50  & 480x640  & COCO & 90.1 \\ \hline

Mask2Former  & ResNet-50  & 480x640  & COCO & 93.5 \\ \hline

MAE~\cite{mae}  & ViT-B + ConvNeXt  & 480x640 & ImageNet-1K & 97.4 \\ \hline

% MultiMAE~\cite{multimae} & ViT-B  + ConvNeXt  & 480x640 & ImageNet-1K & 97.2 \\ \hline

\textbf{SurgDepth} w/ DINOv2  & ViT-B + ConvNeXt  & 480x640 & ImageNet-1K & \textbf{98.1} \\ \hline

\textbf{SurgDepth} w/ DINOv2  & ViT-B + Segmenter  & 480x640 & ImageNet-1K & 96.8 \\ \hline

\hline

\hline

\hline


\end{tabular}
}%
\end{table}
